Diver Identification Using Anthropometric Data Ratios for Underwater Multi-Human-Robot Collaboration

Recent advances in efficient design, perception algorithms, and computing hardware have made it possible to create improved human-robot interaction (HRI) capabilities for autonomous underwater vehicles (AUVs). To conduct secure missions as underwater human-robot teams, AUVs require the ability to accurately identify divers. However, this remains an open problem due to divers' challenging visual features, mainly caused by similar-looking scuba gear. In this paper, we present a novel algorithm that can perform diver identification using either pre-trained models or models trained during deployment. We exploit anthropometric data obtained from diver pose estimates to generate robust features that are invariant to changes in distance and photometric conditions. We also propose an embedding network that maximizes inter-class distances in the feature space and minimizes those for the intra-class features, which significantly improves classification performance. Furthermore, we present an end-to-end diver identification framework that operates on an AUV and evaluate the accuracy of the proposed algorithm. Quantitative results in controlled-water experiments show that our algorithm achieves a high level of accuracy in diver identification.

==> diverID_bibitem.tex <==
\bibitem{bingham2010robotic}Bingham, B., Foley, B., Singh, H., Camilli, R., Delaporta, K., Eustice, R. and Others. Robotic Tools for Deep Water Archaeology: Surveying an Ancient Shipwreck with an Autonomous Underwater Vehicle. {\em Journal Of Field Robotics (JFR)}. vol.~{27}, 702-717 (2010)
\bibitem{edge2020design}Edge, C., Enan, S. S., Fulton, M., Hong, J., Mo, J., Barthelemy, K., Bashaw, H., Kallevig, B., Knutson, C., Orpen, K. and Sattar, J. Design and Experiments with LoCO AUV: A Low Cost Open-Source Autonomous Underwater Vehicle*. {\em 2020 IEEE/RSJ International Conference On Intelligent Robots And Systems (IROS)}. pp. 1761-1768 (2020)
\bibitem{bayat2017environmental}Bayat, B., Crasta, N., Crespi, A., Pascoal, A. and Ijspeert, A. Environmental Monitoring using Autonomous Vehicles: A Survey of Recent Searching Techniques. {\em Current Opinion In Biotechnology}. vol.~{45} pp. 76-84 (2017)
\bibitem{islam2019diverfollowing}Islam, M., Fulton, M. and Sattar, J. Toward a Generic Diver-Following Algorithm: Balancing Robustness and Efficiency in Deep Visual Detection. {\em IEEE Robotics And Automation Letters}. vol.~{4}, 113-120 (2019)
% \bibitem{chatzimichali2021towardprivacy}Chatzimichali, A., Harrison, R. and Chrysostomou, D. Toward privacy-sensitive human–robot interaction: Privacy terms and human–data interaction in the personal robot era. {\em Paladyn, Journal Of Behavioral Robotics}. vol.~{12}, 160-174 (2021)
% \bibitem{r2cvm}Enan, S. S., Fulton, M. and Sattar, J. Robotic Detection of a Human-Comprehensible Gestural Language for Underwater Multi-Human-Robot Collaboration. {\em 2022 IEEE/RSJ International Conference On Intelligent Robots And Systems (IROS)}. pp. 3085-3092 (2022)
\bibitem{mivskovic2016human}Mišković, N., Egi, M., Nad, D., Pascoal, A., Sebastiao, L. and Bibuli, M. Human-Robot Interaction Underwater: Communication and Safety Requirements. {\em 2016 IEEE Third Underwater Communications And Networking Conference (UComms)}. pp. 1-5 (2016)
\bibitem{bengio2017deep}Bengio, Y., Goodfellow, I. and Courville, A. Deep learning. (MIT press Cambridge, MA, USA, 2017)
\bibitem{de2020realtime}De Langis, K. and Sattar, J. Real-Time Multi-Diver Tracking and Re-identification for Underwater Human-Robot Collaboration. {\em 2020 IEEE International Conference On Robotics And Automation (ICRA)}. pp. 11140-11146 (2020)
\bibitem{adroc}Fulton, M., Hong, J. and Sattar, J. Using Monocular Vision and Human Body Priors for AUVs to Autonomously Approach Divers. {\em 2022 International Conference On Robotics And Automation (ICRA)}. pp. 1076-1082 (2022)
\bibitem{xia2019visual}Xia, Y. and Sattar, J. Visual Diver Recognition for Underwater Human-Robot Collaboration. {\em 2019 International Conference On Robotics And Automation (ICRA)}. pp. 6839-6845 (2019)
\bibitem{hong2020visual}Hong, J., Enan, S. S., Morse, C. and Sattar, J. Visual Diver Face Recognition for Underwater Human-Robot Interaction. {\em ArXiv Preprint ArXiv:2011.09556}. (2020)
\bibitem{khan2021gait}Khan, M., Farid, M. and Grzegorzek, M. Vision-based Approaches Towards Person Identification using Gait. {\em Computer Science Review}. vol.~{42} pp. 100432 (2021)
\bibitem{sattar2007fourier}Sattar, J., Bourque, E., Giguere, P. and Dudek, G. Fourier Tags: Smoothly Degradable Fiducial Markers for Use in Human-Robot Interaction. {\em Fourth Canadian Conference On Computer And Robot Vision (CRV '07)}. pp. 165-174 (2007)
\bibitem{islam2018dynamic}Islam, M., Ho, M. and Sattar, J. Dynamic Reconfiguration of Mission Parameters in Underwater Human-Robot Collaboration. {\em 2018 IEEE International Conference On Robotics And Automation (ICRA)}. pp. 6212-6219 (2018)
\bibitem{wilaiprasitporn2020affective}Wilaiprasitporn, T., Ditthapron, A., Matchaparn, K., Tongbuasirilai, T., Banluesombatkul, N. and Chuangsuwanich, E. Affective EEG-Based Person Identification Using the Deep Learning Approach. {\em IEEE Transactions On Cognitive And Developmental Systems}. vol.~{12}, 486-496 (2020)
\bibitem{bae2023digiface}Bae, G., La Gorce, M., Baltrušaitis, T., Hewitt, C., Chen, D., Valentin, J., Cipolla, R. and Shen, J. DigiFace-1M: 1 Million Digital Face Images for Face Recognition. {\em Proceedings Of The IEEE/CVF Winter Conference On Applications Of Computer Vision}. pp. 3526-3535 (2023)
\bibitem{guo2016ms}Guo, Y., Zhang, L., Hu, Y., He, X. and Gao, J. MS-Celeb-1M: A Dataset and Benchmark for Large-Scale Face Recognition. {\em Computer Vision–ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part III 14}. pp. 87-102 (2016)
\bibitem{yang2016wider}Yang, S., Luo, P., Loy, C. and Tang, X. Wider Face: A Face Detection Benchmark. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 5525-5533 (2016)
\bibitem{kortli2020face}Kortli, Y., Jridi, M., Al Falou, A. and Atri, M. Face Recognition Systems: A Survey. {\em Sensors}. vol.~{20}, 342 (2020)
\bibitem{drozdowski2019computational}Drozdowski, P., Rathgeb, C. and Busch, C. Computational Workload in Biometric Identification Systems: An Overview. {\em IET Biometrics}. vol.~{8}, 351-368 (2019)
\bibitem{munsell2012person}Munsell, B., Temlyakov, A., Qu, C. and Wang, S. Person Identification Using Full-Body Motion and Anthropometric Biometrics From Kinect Videos. {\em Computer Vision–ECCV 2012. Workshops And Demonstrations: Florence, Italy, October 7-13, 2012, Proceedings, Part III 12}. pp. 91-100 (2012)
\bibitem{deng2019arcface}Deng, J., Guo, J., Xue, N. and Zafeiriou, S. ArcFace: Additive Angular Margin Loss for Deep Face Recognition. {\em 2019 IEEE/CVF Conference On Computer Vision And Pattern Recognition (CVPR)}. pp. 4685-4694 (2019)
\bibitem{lugaresi2019mediapipe}Lugaresi, C., Tang, J., Nash, H., McClanahan, C., Uboweja, E., Hays, M., Zhang, F., Chang, C., Yong, M., Lee, J. and Others. MediaPipe: A Framework for Building Perception Pipelines. {\em ArXiv Preprint ArXiv:1906.08172}. (2019)
\bibitem{mathis2018deeplabcut}Mathis, A., Mamidanna, P., Cury, K., Abe, T., Murthy, V., Mathis, M. and Bethge, M. DeepLabCut: Markerless Pose Estimation of User-defined Body Parts with Deep Learning. {\em Nature Neuroscience}. vol.~{21}, 1281-1289 (2018)
\bibitem{trtpose}IOT, N. trt\_pose. {\em GitHub Repository}. (2019), https://github.com/NVIDIA-AI-IOT/trt\_pose
\bibitem{openpose}Cao, Z., Simon, T., Wei, S. and Sheikh, Y. Realtime Multi-Person 2D Pose Estimation Using Part Affinity Fields. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition (CVPR)}. (2017,7)
\bibitem{gordon1989anthropometric}Gordon, C., Churchill, T., Clauser, C., Bradtmiller, B., McConville, J., Tebbetts, I. and Walker, R. Anthropometric Survey of US Army Personnel: Summary Statistics, Interim Report for 1988. (Anthropology Research Project Inc Yellow Springs OH,1989)
\bibitem{yang2006distance}Yang, L. and Jin, R. Distance Metric Learning: A Comprehensive Survey. {\em Michigan State University}. vol.~{2}, 4 (2006)
\bibitem{schroff2015facenet}Schroff, F., Kalenichenko, D. and Philbin, J. FaceNet: A Unified Embedding for Face Recognition and Clustering. {\em Proceedings Of The IEEE Conference On Computer Vision And Pattern Recognition}. pp. 815-823 (2015)
\bibitem{peterson2009k}Peterson, L. K-Nearest Neighbor. {\em Scholarpedia}. vol.~{4}, 1883 (2009)
\bibitem{noble2006support}Noble, W. What Is a Support Vector Machine?. {\em Nature Biotechnology}. vol.~{24}, 1565-1567 (2006)
% \bibitem{lin2014micoft}Lin, T., Maire, M., Belongie, S., Hays, J., Perona, P., Ramanan, D., Dollár, P. and Zitnick, C. Microsoft COCO: Common Objects in Context. {\em Computer Vision–ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part V 13}. pp. 740-755 (2014)
\bibitem{wang2020deep}Wang, J., Sun, K., Cheng, T., Jiang, B., Deng, C., Zhao, Y., Liu, D., Mu, Y., Tan, M., Wang, X. and Others. Deep High-Resolution Representation Learning for Visual Recognition. {\em IEEE Transactions On Pattern Analysis And Machine Intelligence}. vol.~{43}, 3349-3364 (2020)
\bibitem{andersson2015person}Andersson, V. and Araujo, R. Person Identification Using Anthropometric and Gait Data from Kinect Sensor. {\em Proceedings Of The AAAI Conference On Artificial Intelligence}. vol.~{29} (2015)
\bibitem{bertillon1896signaletic}Bertillon, A. Signaletic Instructions, including the Theory and Practice of Anthropometrical Identification. {\em Nature}. pp. 569-570 (1896,10)
\bibitem{quigley2009ros}Quigley, M., Conley, K., Gerkey, B., Faust, J., Foote, T., Leibs, J., Wheeler, R., Ng, A. and Others. ROS: An Open-Source Robot Operating System. {\em ICRA Workshop On Open Source Software}. vol.~{3} pp. 5 (2009)
\bibitem{van2008visualizing}Maaten, L. and Hinton, G. Visualizing Data using t-SNE.. {\em Journal Of Machine Learning Research}. vol.~{9} (2008)
\bibitem{ruder2016overview}Ruder, S. An overview of gradient descent optimization algorithms. {\em ArXiv Preprint ArXiv:1609.04747}. (2016)
\bibitem{pedregosa2011scikit}Pedregosa, F., Varoquaux, G., Gramfort, A., Michel, V., Thirion, B., Grisel, O., Blondel, M., Prettenhofer, P., Weiss, R., Dubourg, V. and Others. Scikit-learn: Machine Learning in Python. {\em The Journal Of Machine Learning Research}. vol.~{12} pp. 2825-2830 (2011)
\bibitem{paszke2019pytorch}Paszke, A., Gross, S., Massa, F., Lerer, A., Bradbury, J., Chanan, G., Killeen, T., Lin, Z., Gimelshein, N., Antiga, L., Desmaison, A., Kopf, A., Yang, E., DeVito, Z., Raison, M., Tejani, A., Chilamkurthy, S., Steiner, B., Fang, L., Bai, J. and Chintala, S. PyTorch: An Imperative Style, High-Performance Deep Learning Library. {\em Advances In Neural Information Processing Systems}. pp. 8024-8035 (2019)
\bibitem{nise2000pid}Nise, N. S. Control Systems Engineering. (John Wiley \& Sons, Inc., 3rd. ed., USA, 2000)

==> figs/exp_fig2.tex <==
\begin{figure*}  
    % \vspace{0mm}
    \centering
    % \scalebox{0.75}{\input{figs/id_method.tex}}
    \includegraphics[width=\linewidth]{images/acc.pdf}
    \caption{Average accuracy from our experiments: (Top row): average accuracy for a specific number of test frames across all models, (Bottom row): average accuracy of each model across all frames.}  
    \label{fig:model_accexp}
    \vspace{-4mm}
\end{figure*}


==> figs/exp_fig_bak.tex <==
    \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.475\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/planA_heatmap.jpg}
            % \caption[Network2]%
            % {{\small Network 1}}
            \caption{PlanA}
            \label{fig:intro_rgb}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\linewidth}  
            \centering 
            \includegraphics[width=\linewidth]{images/planA_acc.jpg}
            \caption{PlanA}
            % {{\small Network 2}}    
            \label{fig:intro_seg}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_100heatmap.jpg}
            \caption{PlanB100}
            % {{\small Network 3}}    
            \label{fig:intro_sc}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_100acc.jpg}
            \caption{PlanB100}%
            % {{\small Network 4}}    
            \label{fig:intro_uncertain}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_50heatmap.jpg}
            \caption{PlanB50}
            % {{\small Network 3}}    
            \label{fig:intro_sc}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_50acc.jpg}
            \caption{PlanB50}%
            % {{\small Network 4}}    
            \label{fig:intro_uncertain}
        \end{subfigure}
        \caption{.} 
        % {\small The average and standard deviation of critical parameters: Region R4} 
        \label{fig:experiments}
        \vspace{-4mm}
    \end{figure*}


==> figs/exp_fig_offline.tex <==
    \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.4\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/planA_heatmap.jpg}
            % \caption[Network2]%
            % {{\small Network 1}}
            \caption{PlanA}
            \label{fig:intro_rgb1}
        \end{subfigure}
        % \hfill
        \begin{subfigure}[b]{0.4\linewidth}  
            \centering 
            \includegraphics[width=\linewidth]{images/planA_acc.jpg}
            \caption{PlanA}
            % {{\small Network 2}}    
            \label{fig:intro_seg1}
        \end{subfigure}
        \caption{.} 
        % {\small The average and standard deviation of critical parameters: Region R4} 
        \label{fig:experiments1}
        \vspace{-4mm}
    \end{figure*}


==> figs/exp_fig_test.tex <==
    \begin{figure*}
        \centering
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/planA_heatmap.jpg}
            % \caption[Network2]%
            % {{\small Network 1}}
            \caption{PlanA}
            \label{fig:11}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}  
            \centering 
            \includegraphics[width=\linewidth]{images/planB_50heatmap.jpg}
            \caption{PlanA}
            % {{\small Network 2}}    
            \label{fig:22}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_100heatmap.jpg}
            \caption{PlanB100}
            % {{\small Network 3}}    
            \label{fig:33}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.32\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planA_acc.jpg}
            \caption{PlanB100}%
            % {{\small Network 4}}    
            \label{fig:44}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_50acc.jpg}
            \caption{PlanB50}
            % {{\small Network 3}}    
            \label{fig:55}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}   
            \centering 
            \includegraphics[width=\linewidth]{images/planB_100acc.jpg}
            \caption{PlanB50}%
            % {{\small Network 4}}    
            \label{fig:66}
        \end{subfigure}
        \caption{.} 
        % {\small The average and standard deviation of critical parameters: Region R4} 
        \label{fig:experiments_test}
        \vspace{-4mm}
    \end{figure*}


==> figs/exp_models.tex <==
\begin{table}[t!]
    \vspace{0.2cm}
        \centering
        \caption{Diver Identification Models used for evaluating offline and online frameworks.}
\begin{tabular}{p{0.3\linewidth}p{0.10\linewidth}p{0.10\linewidth}}        
\toprule

 Model Name & Offline & Online \\
\midrule
All\_KNN
 & \checkmark & \checkmark\\
\midrule
Diver\_KNN
 & \checkmark & \checkmark\\
\midrule
All\_SVM
 & \checkmark & \checkmark\\
\midrule
Diver\_SVM
 & \checkmark & \checkmark\\
\midrule
All\_NN\_KNN
 & \checkmark & \checkmark\\
\midrule
Diver\_NN\_KNN
 & \checkmark & \checkmark\\
\midrule
All\_NN\_SVM
 & \checkmark & \checkmark\\
\midrule
Diver\_NN\_SVM
 & \checkmark & \checkmark\\
\midrule
All\_NN
 & \checkmark & -\\
\midrule
Diver\_NN
 & \checkmark & -\\
% Layer 2
%  & Linear. $(1024, 512)$; Leaky ReLU; BN; \\
% \midrule
% Layer 3
%  & Linear. $(512, 256)$; Leaky ReLU; BN; \\
% \midrule
% Layer 4
%  & Linear. $(256, 16)$ \\
 \bottomrule
\end{tabular}
    \label{tab:expmodels}
    \vspace{-0mm}
        \end{table}

==> figs/jds_tab.tex <==
\begin{table}[t!]
    % \vspace{0.2cm}
        \centering
        \caption{Euclidean distances between the listed pairs are used to calculate the corresponding anthropometric data (AD).}
\begin{tabular}{p{0.1\linewidth}p{0.50\linewidth}}        
\toprule
\textbf{AD No.}
 & \textbf{Pairs} \\
\midrule
1
 & (left shoulder, right shoulder) \\
\midrule
2
 & (left shoulder, left hip) \\
\midrule
3
 & (left shoulder, left elbow) \\
\midrule
4
 & (left elbow, left wrist) \\
\midrule
5
 &  (right shoulder, right hip)\\
\midrule
6
 &  (right shoulder, right elbow)\\
\midrule
7
 &  (right elbow, right wrist)\\
\midrule
8
 &  (left hip, right hip)\\
\midrule
9
 &  (left hip, left knee)\\
\midrule
10
 &  (right hip, right knee)\\
 \bottomrule
\end{tabular}
    \label{tab:jds}
    \vspace{-0mm}
        \end{table}

==> figs/method_models.tex <==
\begin{table}[t!]
    \vspace{0.2cm}
        \centering
        \caption{Diver Identification Models used for evaluating offline and online frameworks.}
\begin{tabular}{p{0.3\linewidth}p{0.20\linewidth}p{0.20\linewidth}}        
\toprule

 Model Name & Embedding & Classification \\
\midrule
All\_KNN 
& - & KNN \\
\midrule
Diver\_KNN
& - & KNN \\
\midrule
All\_SVM
& - & SVM \\
\midrule
Diver\_SVM
& - & SVM \\
\midrule
All\_NN\_KNN
& NN & KNN \\
\midrule
Diver\_NN\_KNN
& NN & KNN \\
\midrule
All\_NN\_SVM
& NN & SVM \\
\midrule
Diver\_NN\_SVM
& NN & SVM \\
\midrule
All\_NN
& NN & NN \\
\midrule
Diver\_NN
& NN & NN \\
% Layer 2
%  & Linear. $(1024, 512)$; Leaky ReLU; BN; \\
% \midrule
% Layer 3
%  & Linear. $(512, 256)$; Leaky ReLU; BN; \\
% \midrule
% Layer 4
%  & Linear. $(256, 16)$ \\
 \bottomrule
\end{tabular}
    \label{tab:models}
    \vspace{-0mm}
        \end{table}

==> figs/tab_results_grad.tex <==
\newcommand*{\MinNumber}{0.0}%
\newcommand*{\MidNumber}{0.003} %
\newcommand*{\MaxNumber}{0.008}%
\definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}
\definecolor{darkseagreen}{rgb}{0.56, 0.74, 0.56}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{gray(x11gray)}{rgb}{0.75, 0.75, 0.75}

%Apply the gradient macro
\newcommand{\ApplyGradient}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MaxNumber - #1)/(\MaxNumber-\MinNumber),100.0),0.00)} %
            \hspace{-2mm}\colorbox{white!\PercentColor!red}{#1}\hspace{-1.7mm}
}
\newcommand{\ApplyGradientX}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(3.952 - #1)/(3.952-0.050),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bittersweet}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientY}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.940 - #1)/(1.940-0.025),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!darkseagreen}{#1}\hspace{-1.4mm}
}
\newcommand{\ApplyGradientZ}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(0.008 - #1)/(0.008-0.003),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bleudefrance}{#1}\hspace{-1.4mm}
}
\newcommand{\ApplyGradientXX}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(5.871 - #1)/(5.871-0.419),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bittersweet}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientYY}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(5.990 - #1)/(5.990-0.090),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!darkseagreen}{#1}\hspace{-1.4mm}
}
\newcommand{\ApplyGradientZZ}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(0.031 - #1)/(0.031-0.002),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bleudefrance}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(19.694 - #1)/(19.694-0.514),100.0),0.00)} %
            \hspace{-1.2mm}\colorbox{white!\PercentColor!gray(x11gray)}{#1}\hspace{-1.2mm}
}
\newcommand{\ApplyGradientVV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.82882 - #1/100)/(1.82882-0.00665),100.0),0.00)} %
            \hspace{-1.3mm}\colorbox{white!\PercentColor!gray(x11gray)}{#1}\hspace{-1.1mm}
}
\newcommand{\ApplyGradientVVV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.82882 - #1/100)/(1.82882-0.00665),100.0),0.00)} %
            \hspace{-2mm}\colorbox{white!\PercentColor!gray(x11gray)}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientVVVV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.82882 - #1/100)/(1.82882-0.00665),100.0),0.00)} %
            \hspace{-1.3mm}\colorbox{white!\PercentColor!gray}{#1}\hspace{-1.1mm}
}
% \newcommand{\ApplyGradientV}[1]{%
%             \pgfmathsetmacro{\PercentColor}{max(min(100.0*(19.694 - #1)/(19.694-0.514),100.0),0.00)} %
%             \hspace{-1.8mm}\colorbox{white!\PercentColor!gray}{#1}\hspace{-1.9mm}
% }
% \newcommand{\ApplyGradientVV}[1]{%
%             \pgfmathsetmacro{\PercentColor}{max(min(100.0*(182.882 - #1)/(182.882-0.665),100.0),0.00)} %
%             \hspace{-2.0mm}\colorbox{white!\PercentColor!gray}{#1}\hspace{-1.9mm}
% }

% \newcommand{\ApplyGradient2}[1]{%
%             \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidNumber - #1)/(\MidNumber-\MinNumber),100.0),0.00)} %
%             \hspace{-0.33em}\colorbox{white!\PercentColor!red}{#1}
% }
\newcolumntype{G}{p{0.03\textwidth}>{\collectcell\ApplyGradient}c<{\endcollectcell}}
\newcolumntype{H}{>{\scriptsize\collectcell\ApplyGradient}c<{\endcollectcell}}
\newcolumntype{X}{>{\scriptsize\collectcell\ApplyGradientX}c<{\endcollectcell}}
\newcolumntype{Y}{>{\scriptsize\collectcell\ApplyGradientY}c<{\endcollectcell}}
\newcolumntype{Z}{>{\scriptsize\collectcell\ApplyGradientZ}c<{\endcollectcell}}
\newcolumntype{Q}{>{\scriptsize\collectcell\ApplyGradientXX}c<{\endcollectcell}}
\newcolumntype{R}{>{\scriptsize\collectcell\ApplyGradientYY}c<{\endcollectcell}}
\newcolumntype{S}{>{\scriptsize\collectcell\ApplyGradientZZ}c<{\endcollectcell}}
\newcolumntype{T}{>{\scriptsize\collectcell\ApplyGradientV}c<{\endcollectcell}}
\newcolumntype{U}{>{\scriptsize\collectcell\ApplyGradientVV}c<{\endcollectcell}}
\newcolumntype{I}{>{\scriptsize\collectcell\ApplyGradientVVV}c<{\endcollectcell}}
\newcolumntype{J}{>{\scriptsize\collectcell\ApplyGradientVVVV}c<{\endcollectcell}}

% \renewcommand{\arraystretch}{0}
\setlength{\fboxsep}{1mm}

\newcolumntype{A}{>{\scriptsize\centering}p{0.04\textwidth}}
\newcolumntype{B}{p{0.2\textwidth}}
\newcolumntype{C}{>{\scriptsize\centering}p{0.03\textwidth}}
\newcolumntype{D}{>{\scriptsize\centering\arraybackslash}p{0.04\textwidth}}
\newcolumntype{E}{>{\scriptsize\centering}p{0.045\textwidth}}
\newcolumntype{F}{>{\scriptsize\centering}p{0.059\textwidth}}
\begin{table*}[t!]
{
\centering
\footnotesize
\caption{Localization performance evaluation for an AUV; bathymetry data from the MN DNR.}
\setlength\belowcaptionskip{-0pt}
%   \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
  \begin{tabular}{|C|A|F|C|C|C|A|A|A|F|C|C|C|A|A|D|}
  % \begin{tabular}{|C|A|r*{3}{G}|C|A|A|A|F|C|C|C|A|A|D|}
%   \begin{tabular}{p{0.2\textwidth}*{16}{>{\centering\arraybackslash}}
  \hline
  \multirow{3}{*}{Lake} & \multirow{3}{*}{Method} & \multicolumn{7}{c|}{Linear motion model} & \multicolumn{7}{c|}{Mixed motion model} \\ \cline{3-16}
  
%   & & & & & & & & & & & & & & & \\
%   & & & & & & & & & & & & & & & \\
  
  
  & & \multirow{2}{*}{\makecell{Iteration\\Time ($ms$)}} & \multicolumn{3}{c|}{$RMSE(m)$} & \multicolumn{3}{c|}{$RMSE(\%)$ w.r.t $vel$} & \multirow{2}{*}{\makecell{Iteration\\ Time($ms$)}} & \multicolumn{3}{c|}{$RMSE(m)$} & \multicolumn{3}{c|}{$RMSE(\%)$ w.r.t $vel$} \\ \cline{4-9} \cline{11-16}
  & & & $x$ & $y$ & $z$ & $x$ & $y$ & $z$ & & $x$ & $y$ & $z$ & $x$ & $y$ & $z$  \\ \hline
\end{tabular}
}
\scriptsize
{\centering
\begin{tabular}{|C|A|F|X|Y|Z|T|T|T|F|Q|R|S|U|I|J|}
  Bde. & EKF & 
  20.5 &0.151 & 0.309 & 0.005 & 0.863 & 5.831 & 2.683 &
  20.1 & 5.040 & 5.990 & 0.016 & 53.509 & 182.882 & 8.683\\
  Bde. & UKF &
  0.3& 0.185 & 0.035 & 0.003 & 1.087 & 0.666 & 1.534&
  0.3& 1.786 &	3.488 &	0.019 & 33.166 & 110.868 & 12.082 \\
  Bde. & PF &
  115.0 & 0.395 & 0.540 &0.006 &2.492 & 10.286 & 3.861&
  113.1 & 0.906 &	3.000 &	0.009 & 15.796 & 88.855 & 5.816 \\
  Bde. & MPF &
  61.3 & 0.200 &0.041 & 0.003 & 1.277 & 0.933 & 2.332 &
  62.3 & 1.801 &	3.510 & 0.003 & 33.475 & 112.669 & 1.615  \\ \hline
  
  Nok. & EKF &
  24.0 & 0.349 & 0.295 & 0.004 & 1.523 &	2.687 & 1.831 &
  22.3 & 2.007 & 1.282 &	0.004 & 10.530 & 12.605 & 2.254\\
  Nok. & UKF &
  0.3 & 3.952 & 1.940 & 0.031 & 18.857 & 18.523 & 19.373 &
  0.3 & 5.871 &	2.908 & 0.031 & 32.075 & 31.783&	19.110\\
  Nok. & PF &
  113.9 & 0.553 & 0.182 & 0.007 & 2.623 & 1.667 &	4.465 &
  115.0 & 3.437 & 2.016 &	0.008 & 19.068 & 22.464 & 5.311\\
  Nok. & MPF &
  61.1 & 0.216 & 0.055 & 0.003 & 0.931 & 0.503 & 1.582 &
  62.3 & 2.806 & 1.378 & 0.002 & 15.462 & 15.188 & 1.470\\ \hline

  Hia. & EKF &
  3.0 & 0.289 & 0.240 & 0.004 & 2.337 &	4.233 & 1.111 &
  2.9 & 0.641 &	0.330 & 0.004 & 5.320 & 5.727 & 1.121 \\
  Hia. & UKF &
  0.3 & 0.121 &	0.037 &	0.004 & 1.020 &	0.692 & 1.001 &
  0.3 &0.708 & 0.345 & 0.004 & 4.965 & 4.912 & 1.125\\
  Hia. & PF &
  112.5 & 0.472 & 0.272 &	0.004 & 4.224 &	4.709 &	1.334 &
 112.4 & 1.073 & 0.509 & 0.006 & 8.539 & 8.873 &	1.728\\
  Hia. & MPF &
  62.5 & 0.089 &	0.022 & 0.003 & 0.714 &	0.390 & 0.926 &
  62.3 & 0.711 & 0.346 & 0.005 & 4.988 & 4.930 &	1.417\\ \hline

  Har. & EKF &
  17.4 & 0.236 &	0.152 &	0.003 & 1.405 &	1.5170 & 0.925 &
  17.2 & 1.385 &	0.822 &	0.003 & 9.367 &	9.844 & 0.856 \\
  Har. & UKF &
  0.3 &  0.812 &	0.406 &	0.003 & 6.820 &	6.931 &	1.222 &
  0.3 &  1.610 &	0.810 &	0.003 & 11.460 & 11.088 & 1.077\\
  Har. & PF &
  112.9 & 0.290 &	0.452 &	0.005 & 1.640 & 5.128 & 1.668 &
  112.7 & 1.665 &	1.372 &	0.006 & 10.496 & 15.660 & 1.708\\
  Har. & MPF &
  61.3 & 0.143 &	0.035 &	0.003 & 0.749 &	0.401 & 0.891 &
  62.2 & 2.103 &	1.058 & 0.003 & 11.550 & 11.192 & 1.034 \\ \hline
  
  Tur. & EKF &
  24.7 & 0.355 &	0.211 & 0.003 &  3.090 & 1.993 & 0.831 &
  22.4 & 0.479 & 0.347 &	0.004 & 3.366 &	12.087 & 0.930\\
  Tur. & UKF &
  0.3 & 0.128 &	0.075 &	0.004 & 1.126 &	0.711 & 1.221 &
  0.3 & 0.419 &	0.090 & 0.004 & 2.983 &	3.006 &	0.966\\
  Tur. & PF &
  112.5 & 0.516 & 0.251 &	0.006 & 4.815 & 2.399 &	1.893 &
  115.6 & 0.948 & 0.723 & 0.006 & 7.521 & 28.647 & 1.816\\
  Tur. & MPF &
  62.0 & 0.091 &	0.041 & 0.003 & 0.775 & 0.366 & 0.763&
  62.2 & 0.451 &	0.098 & 0.003 & 3.210 &	3.295 & 0.864\\ \hline

  How. & EKF &
  94.4 & 0.423 & 0.315 & 0.007 & 4.010 &	2.447 &	1.715 &
  84.0 & 1.622 & 0.971 & 0.006 & 12.304 & 8.386 & 1.747\\
  How. & UKF &
  0.3 &0.115 & 0.074 & 0.005 & 0.991 & 0.640 & 1.351 &
  0.3 &1.771 & 1.807 & 0.006 & 13.722 & 14.078 & 1.789\\
  How. & PF &
  113.2 & 0.745 &	0.747 &	0.008 & 6.478 &	7.003 &	2.330 &
  115.5 & 1.730 & 1.820 & 0.007 & 13.379 & 14.387 &  1.971\\
  How. & MPF &
  61.4 & 0.127 &	0.076 & 0.006 & 1.135 & 0.719 & 1.809 &
  61.3 & 1.831 &	1.867 & 0.004 & 14.265 & 14.617 & 1.180\\ \hline
  
  Wav. & EKF &
  37.1 & 0.154 & 0.100 & 0.004 & 2.877 &	1.609 & 0.985 &
  40.5 & 0.649 &	0.572 & 0.004 & 6.526 &	9.100 & 1.034\\
  Wav. & UKF &
  0.3 &0.050 & 0.025 & 0.004 & 0.853 & 0.456 & 1.246 &
  0.3 &1.040 & 0.710 & 0.004 & 10.464 & 10.885 & 1.245\\
  Wav. & PF &
  115.5 & 0.309 & 1.113 & 0.006 & 5.666 & 19.694 & 1.770 &
  116.3 & 0.995 & 0.564 & 0.006 & 11.545 & 9.238 & 1.805\\
  Wav. & MPF &
  61.7 & 0.059 &	0.033 & 0.006& 1.029 & 0.612 & 1.727 &
  61.5 & 1.057 & 0.721 & 0.005 & 10.670 & 11.084 & 1.515\\ \hline
  
  Pul. & EKF &
  69.8 & 0.118 & 0.103 & 0.004 & 1.990 & 1.775 & 0.906 &
  62.1 & 2.120 &	2.346 & 0.005 & 17.248 & 16.117 & 1.546\\
  Pul. & UKF &
  0.3 &0.055 & 0.028 & 0.003 & 0.936 & 0.514 & 0.792 &
  0.3 & 3.781 & 3.708 & 0.009 & 25.876 & 25.425 & 2.775\\
  Pul. & PF &
  113.3 & 0.563 &	0.865 & 0.004 & 10.618 & 16.022 & 1.087 &
  113.9 & 2.951 & 2.978 & 0.006 & 20.136 & 20.368 & 1.679\\
  Pul. & MPF &
  61.8 & 0.076 & 0.052 & 0.006 & 1.411 &	1.003 &	1.930 &
  61.3 & 3.764 & 3.691 & 0.002 & 25.756 & 25.302 & 0.665\\ \hline
\end{tabular}
}
% \vspace{-5mm}
\label{tb:resulteval_new}
\\
\footnotesize{The intensity of each color is proportional to the error. Red, green and blue colors are used for the x, y, and z-axis, respectively. Grey color represents the percentage errors across all the axis.}
\end{table*}


==> figs/tab_test.tex <==
\newtoggle{inTableHeader}% Track if still in header of table
\toggletrue{inTableHeader}% Set initial value
\newcommand*{\StartTableHeader}{\global\toggletrue{inTableHeader}}%
\newcommand*{\EndTableHeader}{\global\togglefalse{inTableHeader}}%

% Redefine tabular to initialize \StartTableHeader at start and end
\let\OldTabular\tabular%
\let\OldEndTabular\endtabular%
\renewenvironment{tabular}{\StartTableHeader\OldTabular}{\OldEndTabular\StartTableHeader}%



\newcommand*{\MinNumber}{0.0}%
\newcommand*{\MidNumber}{0.5} %
\newcommand*{\MaxNumber}{1.0}%
\definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}
\definecolor{darkseagreen}{rgb}{0.56, 0.74, 0.56}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{gray(x11gray)}{rgb}{0.75, 0.75, 0.75}

%Apply the gradient macro
\newcommand{\ApplyGradient}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MaxNumber - #1)/(\MaxNumber-\MinNumber),100.0),0.00)} %
            \hspace{-2mm}\colorbox{white!\PercentColor!red}{#1}\hspace{-1.7mm}
}
\newcommand{\ApplyGradientX}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(3.952 - #1)/(3.952-0.050),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bittersweet}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientY}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.940 - #1)/(1.940-0.025),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!darkseagreen}{#1}\hspace{-1.4mm}
}
\newcommand{\ApplyGradientZ}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(0.008 - #1)/(0.008-0.003),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bleudefrance}{#1}\hspace{-1.4mm}
}
\newcommand{\ApplyGradientXX}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(5.871 - #1)/(5.871-0.419),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bittersweet}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientYY}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(5.990 - #1)/(5.990-0.090),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!darkseagreen}{#1}\hspace{-1.4mm}
}
\newcommand{\ApplyGradientZZ}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(0.031 - #1)/(0.031-0.002),100.0),0.00)} %
            \hspace{-1.5mm}\colorbox{white!\PercentColor!bleudefrance}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(19.694 - #1)/(19.694-0.514),100.0),0.00)} %
            \hspace{-1.2mm}\colorbox{white!\PercentColor!gray(x11gray)}{#1}\hspace{-1.2mm}
}
\newcommand{\ApplyGradientVV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.82882 - #1/100)/(1.82882-0.00665),100.0),0.00)} %
            \hspace{-1.3mm}\colorbox{white!\PercentColor!gray(x11gray)}{#1}\hspace{-1.1mm}
}
\newcommand{\ApplyGradientVVV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.82882 - #1/100)/(1.82882-0.00665),100.0),0.00)} %
            \hspace{-2mm}\colorbox{white!\PercentColor!gray(x11gray)}{#1}\hspace{-1.5mm}
}
\newcommand{\ApplyGradientVVVV}[1]{%
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(1.82882 - #1/100)/(1.82882-0.00665),100.0),0.00)} %
            \hspace{-1.3mm}\colorbox{white!\PercentColor!gray}{#1}\hspace{-1.1mm}
}
% \newcommand{\ApplyGradientV}[1]{%
%             \pgfmathsetmacro{\PercentColor}{max(min(100.0*(19.694 - #1)/(19.694-0.514),100.0),0.00)} %
%             \hspace{-1.8mm}\colorbox{white!\PercentColor!gray}{#1}\hspace{-1.9mm}
% }
% \newcommand{\ApplyGradientVV}[1]{%
%             \pgfmathsetmacro{\PercentColor}{max(min(100.0*(182.882 - #1)/(182.882-0.665),100.0),0.00)} %
%             \hspace{-2.0mm}\colorbox{white!\PercentColor!gray}{#1}\hspace{-1.9mm}
% }

% \newcommand{\ApplyGradient2}[1]{%
%             \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidNumber - #1)/(\MidNumber-\MinNumber),100.0),0.00)} %
%             \hspace{-0.33em}\colorbox{white!\PercentColor!red}{#1}
% }
\newcolumntype{G}{p{0.03\textwidth}>{\collectcell\ApplyGradient}c<{\endcollectcell}}
\newcolumntype{H}{>{\scriptsize\collectcell\ApplyGradient}c<{\endcollectcell}}
\newcolumntype{X}{>{\scriptsize\collectcell\ApplyGradientX}c<{\endcollectcell}}
\newcolumntype{Y}{>{\scriptsize\collectcell\ApplyGradientY}c<{\endcollectcell}}
\newcolumntype{Z}{>{\scriptsize\collectcell\ApplyGradientZ}c<{\endcollectcell}}
\newcolumntype{Q}{>{\scriptsize\collectcell\ApplyGradientXX}c<{\endcollectcell}}
\newcolumntype{R}{>{\scriptsize\collectcell\ApplyGradientYY}c<{\endcollectcell}}
\newcolumntype{S}{>{\scriptsize\collectcell\ApplyGradientZZ}c<{\endcollectcell}}
\newcolumntype{T}{>{\scriptsize\collectcell\ApplyGradientV}c<{\endcollectcell}}
\newcolumntype{U}{>{\scriptsize\collectcell\ApplyGradientVV}c<{\endcollectcell}}
\newcolumntype{I}{>{\scriptsize\collectcell\ApplyGradientVVV}c<{\endcollectcell}}
\newcolumntype{J}{>{\scriptsize\collectcell\ApplyGradientVVVV}c<{\endcollectcell}}

% \renewcommand{\arraystretch}{0}
\setlength{\fboxsep}{1mm}

\newcolumntype{A}{>{\scriptsize\centering}p{0.04\textwidth}}
\newcolumntype{B}{p{0.2\textwidth}}
\newcolumntype{C}{>{\scriptsize\centering}p{0.03\textwidth}}
\newcolumntype{D}{>{\scriptsize\centering\arraybackslash}p{0.04\textwidth}}
\newcolumntype{E}{>{\scriptsize\centering}p{0.045\textwidth}}
\newcolumntype{F}{>{\scriptsize\centering}p{0.059\textwidth}}



% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{cllll}
% \multicolumn{1}{l}{\multirow{2}{*}{}} & \multirow{2}{*}{\# of Frames} & \multicolumn{3}{l}{Model Accuracy}  \\
% \multicolumn{1}{l}{}                  &                               & Offline & Online (50) & Online(100) \\
% \multirow{10}{*}{All\_NN}             & 10                            &         &             &             \\
%                                       & 20                            &         &             &             \\
%                                       & 30                            &         &             &             \\
%                                       & 40                            &         &             &             \\
%                                       & 50                            &         &             &             \\
%                                       & 60                            &         &             &             \\
%                                       & 70                            &         &             &             \\
%                                       & 80                            &         &             &             \\
%                                       & 90                            &         &             &             \\
%                                       & 100                           &         &             &             \\
% \multicolumn{1}{l}{}                  &                               &         &             &             \\
% \multicolumn{1}{l}{}                  &                               &         &             &            
% \end{tabular}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{lllllllllllH}
\multirow{2}{*}{Models}       &              & \multicolumn{10}{l}{Number of Frames}            \\
                              &              & 10 & 20 & 30 & 40 & 50 & 60 & 70 & 80 & 90 & 100\\ \hline 
\multirow{3}{*}{All\_NN}      & Offline      &    &    &    &    &    &    &    &    &    &  0.3   \\
                              & Online (50)  &    &    &    &    &    &    &    &    &    &  0.5  \\
                              & Online (100) &    &    &    &    &    &    &    &    &    &  1.0   \\
\multirow{3}{*}{All\_NN\_KNN} & Offline      &    &    &    &    &    &    &    &    &    &   0.0  \\
                              & Online (50)  &    &    &    &    &    &    &    &    &    &    0.0\\
                              & Online (100) &    &    &    &    &    &    &    &    &    &    0.0 \\
                              &              &    &    &    &    &    &    &    &    &    &    0.0
\end{tabular}
\end{table*}

==> figs/tab_test2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{Comparison of the diver identification accuracy of the proposed system across $10$ different models. The darker colors represent higher accuracy.}
\begin{tabular}{@{}cccccccccccccccc@{}}
\toprule
                 % & \multicolumn{15}{c}{Accuracy}                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \midrule
 \textbf{Model Name}                 & \multicolumn{3}{c}{\textbf{All\_KNN}}                                                               & \multicolumn{3}{c}{\textbf{Diver\_KNN}}                                                             & \multicolumn{3}{c}{\textbf{All\_SVM}}                                                               & \multicolumn{3}{c}{\textbf{Diver\_SVM}}                                                             & \multicolumn{3}{c}{\textbf{All\_NN\_KNN}}                                                           \\
                 \midrule
\textbf{Framework}  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  \\
 \textbf{Number of Frames}                &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}                           & \textbf{100}                          \\
                 \midrule
10               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 \\
20               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 \\
30               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 \\
40               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 \\
50               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 \\
60               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
70               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
80               & \cellcolor[HTML]{F8A102}0.67 & -                         & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
90               & \cellcolor[HTML]{F8A102}0.67 & -                         & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
100              & \cellcolor[HTML]{F8A102}0.67 & \phantom{0.}-\phantom{0.}                         & \phantom{0.}-\phantom{0.} & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \phantom{0.}-\phantom{0.} & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\ \bottomrule
\end{tabular}
\label{tab:results}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\begin{tabular}{@{}cccccccccccccccc@{}}
% \toprule
%                  & \multicolumn{15}{c}{Accuracy}                                                                                                                                                                                                                                                                                                                                                                                \\ \midrule
\textbf{Model Name}                 & \multicolumn{3}{c}{\textbf{Diver\_NN\_KNN}}                                                         & \multicolumn{3}{c}{\textbf{All\_NN\_SVM}}                                                           & \multicolumn{3}{c}{\textbf{Diver\_NN\_SVM}}                                                         & \multicolumn{3}{c}{\textbf{All\_NN}}                               & \multicolumn{3}{c}{\textbf{Diver\_NN}}                             \\
                 \midrule
\textbf{Framework} & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                  & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}}                                 & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}} & \textbf{Offline}                      & \multicolumn{2}{c}{\textbf{Online}} \\
\textbf{Number of Frames}                 &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}                           & \textbf{100}                          &                              & \textbf{50}          & \textbf{100}          &                              & \textbf{50}          & \textbf{100}          \\
                 \midrule
10               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{FFCE93}0.33 & -           & -            \\
20               & 0.00                         & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & 0.00                         & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
30               & 0.00                         & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
40               & 0.00                         & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
50               & 0.00                         & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
60               & 0.00                         & -                            & \cellcolor[HTML]{F8A102}0.67                         & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
70               & 0.00                         & -                            & \cellcolor[HTML]{F8A102}0.67                         & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
80               & 0.00                         & -                            & \cellcolor[HTML]{F8A102}0.67                         & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
90               & 0.00                         & -                            & \cellcolor[HTML]{F8A102}0.67                         & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & -           & -            & \cellcolor[HTML]{F8A102}0.67 & -           & -            \\
100              & 0.00                         & -                            & \cellcolor[HTML]{F8A102}0.67                         & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \phantom{0.}-\phantom{0.}           & \phantom{0.}-\phantom{0.}            & \cellcolor[HTML]{F8A102}0.67 & \phantom{0.}-\phantom{0.}           & \phantom{0.}-\phantom{0.}            \\ \bottomrule
\end{tabular}
\end{table*}

==> figs/tab_test3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\begin{tabular}{@{}cccccccccccccccc@{}}
\toprule
                 & \multicolumn{15}{c}{Accuracy}                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \midrule
                 & \multicolumn{3}{c}{All\_KNN}                                                         & \multicolumn{3}{c}{Diver\_KNN}                                                             & \multicolumn{3}{c}{All\_SVM}                                                         & \multicolumn{3}{c}{Diver\_SVM}                                                             & \multicolumn{3}{c}{All\_NN\_KNN}                                                           \\
Number of Frames & Offline                      & \multicolumn{2}{c}{Online}                            & Offline                      & \multicolumn{2}{c}{Online}                                  & Offline                      & \multicolumn{2}{c}{Online}                            & Offline                      & \multicolumn{2}{c}{Online}                                  & Offline                      & \multicolumn{2}{c}{Online}                                  \\
                 &                              & 50                        & 100                       &                              & 50                           & 100                          &                              & 50                        & 100                       &                              & 50                           & 100                          &                              & 50                           & 100                          \\
10               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 \\
20               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 \\
30               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 \\
40               & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 \\
50               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 & \cellcolor[HTML]{F56B00}1.00 \\
60               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
70               & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
80               & \cellcolor[HTML]{F8A102}0.67 & -                         & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
90               & \cellcolor[HTML]{F8A102}0.67 & -                         & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFCE93}0.33 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFCE93}0.33 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\
100              & \cellcolor[HTML]{F8A102}0.67 & -                         & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{FFFFFF}- & \cellcolor[HTML]{F8A102}0.67 & -                            & \cellcolor[HTML]{F8A102}0.67 & \cellcolor[HTML]{F56B00}1.00 & -                            & \cellcolor[HTML]{F56B00}1.00 \\ \bottomrule
\end{tabular}
\end{table*}

==> src/1introduction_bak.tex <==
\section{Introduction}
In recent years, underwater robotics has advanced significantly, mainly driven by increased onboard computational power, improved perception, and enhanced human-robot interaction (HRI) capabilities of autonomous underwater vehicles (AUVs). 
Such advances allow AUVs to be used in both independent (\eg environmental monitoring~\cite{bayat2017environmental}) and collaborative missions (\eg diver following~\cite{islam2019diverfollowing}). Underwater HRI has the potential to be extended for more advanced human-robot collaborative missions (\eg shipwreck and pipeline inspection~\cite{bingham2010robotic}) where robots can rely on human expertise while reducing risks posed to humans. 

However, there are still challenges that need to be addressed to use HRI capabilities for such missions, and \textit{diver identification} for these missions is one of them. In general, AUVs have limited operating time underwater due to constraints caused by environmental (\eg rapid current and water turbidity) and operational factors (\eg battery time). Taking conflicting instructions from divers can delay and jeopardize missions. For instance, in a multi-diver single-robot collaboration scenario (as shown in Fig.~\ref{fig:intro}), the ability to correctly identify divers would enable the robot to keep each diver's data and instruction separate.
\input{figs/intro_fig.tex}To address the diver identification problem, researchers have proposed fiducial markers~\cite{sattar2007fourier}, unique hand signs~\cite{islam2018dynamic}, acoustic communication devices~\cite{mivskovic2016human}, and other specifically-engineered devices. 
However, with these methods, the diver must carry additional items or memorize unique hand signals, which can add to the already-elevated cognitive and physical burdens. Losing or forgetting such means of identification will compromise the entire mission. To address these issues, recent work~\cite{hong2020visual} uses facial cues to identify different divers by synthetically removing the dive mask and breathing apparatus from their face to compute unique facial features. However, the proposed method requires the collection of diver face data prior to the mission. Also, it can fail due to facial distortion at the edges of the masks and the area surrounding the lips caused by wearing the mask and breathing apparatus. To overcome this problem, an ideal diver identification method must be functional in data-scarce and visually challenging conditions.
% underwater is an inherently challenging domain to develop and test the identification algorithms due to limited access to electromagnetic signals (\eg Wi-Fi) and degraded vision. Additionally, any visual-feature-based identification methods using deep learning models (\eg face identification) show degraded performance. Because scuba gears look similar, divers' faces are heavily obscured by breathing apparatus, and there are not enough data from underwater for the deep learning models to learn visual features via training. 
% Therefore, it is critical to identify divers before starting any interaction. 
% There are multiple factors to this. Underwater is an inherently challenging domain to develop and test the identification algorithms due to limited access to electromagnetic signals (\eg Wi-Fi) and degraded vision. Additionally, any visual-feature-based identification methods using deep learning models (\eg face identification) show degraded performance. Because scuba gears look similar, divers' faces are heavily obscured by breathing apparatus, and there are not enough data from underwater for the deep learning models to learn visual features via training.
\input{figs/id_fig.tex}
% However, underwater is an inherently challenging domain to develop and test the identification algorithms due to limited access to electromagnetic signals (\eg Wi-Fi) and degraded vision. Additionally, any visual-feature-based identification methods using deep learning models (\eg face identification) show degraded performance. Because scuba gears look similar, divers' faces are heavily obscured by breathing apparatus, and there are not enough data from underwater for the deep learning models to learn visual features via training. 
% So, we investigate an identification system where the divers do not need to remember any signs or carry any specialized equipment to be uniquely identified by AUVs. 

% Thus, We aim to address a diver identification problem for AUVs to enable efficient human-robot collaboration missions while addressing the underwater domain challenges and constraints from the previous methods.
In this work, we propose a diver identification framework that uses anthropometric data (AD) of the divers. Our framework can be deployed with either pre-trained models (\textbf{offline framework}) or models that can be trained during deployment (\textbf{online framework}). This allows the AUV to identify divers even if their data is not present in our dataset (\ie identify divers previously unseen by the robot by creating AD models `on-the-fly').
 % The goal of our proposed algorithm is to find a target diver, which will be assigned before the deployment. The offline framework is used when the target diver data is present in our dataset, whereas the online framework is used when we do not have the target diver data before deployment.
This enables efficient human-robot collaborative missions with robust diver identification by addressing the domain-specific challenges underwater and constraints introduced above.
\textit{Anthropometric data} refers to the study of human body measurements, such as the width of shoulders, lengths of the lower and upper arms, and measurement of other limbs or limb sections. 
AD can be captured even if divers' bodies and faces are heavily obscured. However, the AD can change during the identification process, since the distance between the robot and the diver can vary. %, which will introduce variability in the diver's anthropometric data from the robot's perspective. 
Therefore, we propose to use \textit{anthropometric data ratios} (ADRs) instead, to represent divers uniquely, exploiting the property that ADRs will be invariant to the robot-diver distance. 
% To compute the ADRs, we first identify $10$ joint locations on a diver's body using a $2D$ pose estimation algorithm~\cite{wang2020deep}. Second, we filter out the inaccurate poses to compute the AD values from only valid pose data. Finally, we calculate $45$ different ADRs using these values and use them to represent scuba divers in this feature space. 
Through experiments, we demonstrate that these ADR features can be projected into a $16$-d hyperspace where they show better separation. We achieve this by using our proposed embedding network that maximizes inter-class feature distance and minimizes intra-class feature distance, which significantly improves the classification performance. With that, we present a complete diver identification framework for underwater robots to identify divers using only ADR features.

% can form highly separable clusters in a $16$-dimensional hyperspace. We use an embedding network to generate this lower dimensional feature embedding that maximizes inter-class distance and minimizes intra-class distance. With that, we present a complete diver identification framework for underwater robots to identify divers using only ADR features.
% Through experiments, we show that our proposed embedding network can generate $16$-d features from the ADR features. Also, we demonstrate that this $16$-d feature embedding forms highly separable clusters by maximizing inter-class distances and minimizing intra-class distances. As a result, we improve the identification accuracy with our approach. With that, we present a complete diver identification framework for underwater robots to identify divers using only ADR features.
% Through experiments, we show that ADR features with our embedding network successfully form highly separable inter-class clusters, which subsequently maximizes identification accuracy. With that, we present a complete diver identification framework for underwater robots to identify divers using only ADR features.

In our framework, a robot starts by searching for and then approaching divers for identification. For the offline framework, the robot uses pre-trained models to identify the divers using ADR features generated by pose estimation and feature extraction. For the online framework, the robot collects data first to train models on-the-fly and identifies the divers upon completing the training. Our framework enables the robot to: (1) identify the divers with their known identities using the offline framework when prior data is available, and (2) distinguish the divers with the online framework even if their data is not available to the robot prior to deployment. We evaluate both frameworks with our proposed identification module in a closed-water environment onboard a physical AUV and demonstrate promising results. We make the following contributions in this paper:
\begin{enumerate}
    \item We propose distance and photometric invariant features, called anthropometric data ratios (ADRs), to create unique representations of scuba divers. 
    \item We introduce an embedding network that can project the ADR features to a $16$-d hyperspace where they form highly separable inter-class clusters, resulting in superior classification performance.
    \item We use anthropometric data statistics to filter out erroneous diver pose estimations. 
    \item We propose a diver identification algorithm for underwater robots to use the collected features to train a number of models both offline and online.
    % \item We deploy the proposed algorithm on a physical AUV in a controlled underwater environment and measure the efficacy of the system.
    \item We measure the efficacy of the system on a physical AUV in a closed-water environment.
\end{enumerate}


% Human-robot collaborative missions enable the robots to rely on human expertise, and humans to exploit robotic perception and autonomy, which improves overall task completion efficiency.
% Nevertheless, safety in HRI methods remains an open problem~\cite{chatzimichali2021towardprivacy}, especially when robots are required to take instructions from only a few authorized individuals. 
% One of the contributing factors to this, in the context of underwater HRI (UHRI), is that the robot needs to uniquely identify divers under similar wearables, which poses a significant challenge due to the difficulty in generating distinguishable features just from both their faces and bodies. 
% Additionally, the ever-demanding underwater environment, with water turbidity, rapid currents, and varying lighting conditions, just makes this task even more difficult for the robots. 
% Unable to identify authorized divers can have a severe negative impact on the mission outcome, as this can compromise the overall safety of any underwater mission, especially search-and-rescue and maritime defense operations. 
% Furthermore, in a multi-diver single-robot collaboration scenario (as shown in Fig.~\ref{fig:intro}), the ability to correctly identify divers would enable the robot to keep each diver's data or instruction separate.
% \input{figs/intro_fig.tex}

% Thus, we seek a diver identification algorithm for AUVs to enable secure communication between a diver and the robot. 
% To verify their identity to an AUV, the divers can use fiducial markers~\cite{sattar2007fourier}, unique hand signs~\cite{islam2018dynamic}, acoustic communication device~\cite{mivskovic2016human}, and other specifically-engineered devices. 
% However, with these methods, the diver needs to carry an additional fiducial marker, specialized communication equipment, or remember a unique hand signal for self-identification (or authentication), which can add to the already-elevated cognitive and physical burdens. The markers may also get destroyed or lost during a mission. So, we investigate an identification system where the divers do not need to remember any signs or carry any specialized equipment to be uniquely identified by AUVs. Recent work~\cite{hong2020visual} has shown that facial cues can be used underwater to identify different divers, by synthetically removing the dive mask and breathing apparatus from a diver's face to compute unique facial features. However, the proposed synthetic face generation method can fail because of the complexity of a diver's facial appearance. Since the mask and breathing apparatus introduce facial distortion at the edges of the masks and the area surrounding the lips, respectively, the proposed algorithm has been shown to be unable to remove those distortions. 
% % In addition, prescription scuba masks distort eye information. Therefore, unique facial features can be computed from synthetically generated faces.
% \input{figs/id_fig.tex}

% In this work, we explore if anthropometric data (AD) (\eg \cite{andersson2015person}) can be used to identify divers under similar wearables. 
% \textit{Anthropometric data} refers to the study of human body measurements, such as the width of shoulders, lengths of the lower and upper arms, and measurement of other limbs or limb sections. However, during underwater HRI, the distance between the robot and the diver can vary, which will introduce variability in the diver's anthropometric data from the robot's perspective. Therefore, we propose to use \textit{anthropometric data ratios} (ADRs) instead, to represent divers uniquely, exploiting the property that ADRs will be invariant to the robot-diver distance. To compute the ADRs, we first identify $10$ joint locations on a diver's body using a $2D$ pose estimation algorithm~\cite{wang2020deep}. Second, we filter out the inaccurate poses to compute the AD values from only valid pose data. Finally, we calculate $45$ different ADRs using these values and use them to represent scuba divers in this feature space. Through experiments, we show that the ADRs can form highly separable clusters in a $16$-dimensional hyperspace, which is created by passing these $45$ ADRs through an embedding network. With that, we present a complete \textit{diver identification framework} for underwater robots to identify divers using only ADR features. We test our algorithm, which can be incorporated in both offline and online frameworks, in a controlled underwater pool environment onboard a physical AUV and demonstrate promising results. We make the following contributions in this paper:
% \begin{enumerate}
%     \item We show that the anthropometric data ratios (ADRs) can be used to create unique representation of scuba divers. 
%     \item We also demonstrate that these ratios form highly separable clusters for different divers in a $16$-dimensional hyperspace, by passing these $45$ ADRs through an embedding network.
%     \item We use anthropometric data statistics to filter out erroneous pose estimations. 
%     \item We propose a diverID algorithm for underwater robots to use the collected features to train and classify a number of learning models both online and offline.
%     \item We deploy the proposed algorithm on a physical AUV in a controlled underwater environment and measure the efficacy of the system.
% \end{enumerate}

%% Anthropometric Data Ration (ADR) 
% \lipsum[2-6]


%~\cite{edge2020design}
